Game-Theoretic Malware Detection

Malware attacks are costly. To mitigate against such attacks, organizations deploy malware detection tools that help them detect and eventually resolve those threats. While running only the best available tool does not provide enough coverage of the potential attacks, running all available tools is prohibitively expensive in terms of financial cost and computing resources. Therefore, an organization typically runs a set of tools that maximizes their coverage given a limited budget. However, how should an organization choose that set? Attackers are strategic, and will change their behavior to preferentially exploit the gaps left by a deterministic choice of tools. To avoid leaving such easily-exploited gaps, the defender must choose a random set. In this paper, we present an approach to compute an optimal randomization over size-bounded sets of available security analysis tools by modeling the relationship between attackers and security analysts as a leader-follower Stackelberg security game. We estimate the parameters of our model by combining the information from the VirusTotal dataset with the more detailed reports from the National Vulnerability Database. In an empirical comparison, our approach outperforms a set of natural baselines under a wide range of assumptions.

==> figures/deps.tex <==
\begin{figure}
\centering
    \includegraphics[width=\columnwidth]{resources/CVE_independence.png}
\caption{Tool dependency scores within the VirusTotal dataset} 
\label{fig:dependencies}
\end{figure}

==> figures/new_results_yds_yas.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/yas_line.pdf}
         \caption{$\gamma_a$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/yds_line.pdf}
         \caption{$\gamma_d$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/legend.png}
     \end{subfigure}
        \caption{\revan{Here's an alternate, less busy version of the figure above. Thoughts?}
        \jrw{I like this a lot better, also for figure 1}}
        \label{fig:three graphs}
\end{figure*}


==> figures/results_yds.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{resources/results_yds.png}
    \caption{Expected utility of the defender with $\gamma_a = 1$ and varying $\gamma_d$. We compare our proposed randomized best response (\rbr) to deterministic best response (\dbr) and other baselines, described in \secref{labeldescriptions}. Utilities closer to zero indicate better performance.}
    \label{fig:results_yds}
\end{figure*}

==> figures/rq1.tex <==
\begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{resources/results_all.png}
    \label{fig:results}
\end{subfigure}

==> figures/rq2.tex <==
\begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{resources/results_pdf.png}
    \caption{Only PDF files.}
    \label{fig:results_pdf}
\end{subfigure}

==> resources/mem_use.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
\multicolumn{5}{c}{\textbf{LP Generation}}          \\
\midrule 
\textbf{Budget}   & \textbf{Run 1}   & \textbf{Run 2}    & \textbf{Run 3}  & \textbf{Average}   \\
\midrule
1        & 205,364  & 205,380  & 205,136  & 205,293   \\
2        & 346,787  & 276,396  & 276,968  & 300,050   \\
3        & 5,908,384 & 5,908,396 & 5,908,920 & 5,908,567  \\
\midrule
\multicolumn{5}{c}{\textbf{LP Solve}}  \\
\midrule
\textbf{Budget}   & \textbf{Run 1}   & \textbf{Run 2}    & \textbf{Run 3}  & \textbf{Average}   \\
\midrule
1        & 45,916   & 45,952   & 45,864   & 45,911    \\
2        & 417,180  & 419,768  & 417,132  & 418,027   \\
3        & 7,366,504 & 7,347,268 & 7,369,908 & 7,361,227  \\
\bottomrule
\end{tabular}}
\caption{The memory consumption of generating and solving LP in terms of maximum resident set size (kbytes). \ka{I don't think that this table is the best approach to represent our data.} \ka{are these runs different than the ones in \tabref{table:run_time}?}}
\label{table:mem_use}
\end{table}


==> resources/notes.tex <==
USENIX requires the following formatting rules be followed:
    * Enumerated references (eg: [1] Jain, M., ...), in the order that they are cited in the paper.
    * References should include a link to where readers can access them.
    * Figure text should be as large or larger than the figure's caption text (10px or larger)
    * I didn't find anything about page limits or anything else concerning formatting
    
Other:
* Resources is for figures, figure captions, references, and notes
* Style is for style sheets
* Text is for text content of the paper.

example paper here:
\burl{https://www.usenix.org/sites/default/files/usenix2019_v3.1.pdf}

==> resources/pruning_algorithm.tex <==

\begin{algorithm*}
\caption{Pruning Dominated Schedules}\label{alg:prune_dominated}
\begin{algorithmic}[1]
\Procedure{remove\_dominated}{$S, V, ud, num\_threads$}
    \State $S, ud \ = \ \Call{lexsort}{S, ud}$ \Comment{order ud, S lexicographically by ud} \label{state:lexsort}
    \State $nd\_shared \ = \ S$ \Comment{shared set of non-dominated schedules}
    \For{$i = 0,1, ...,  num\_threads $}
         \State $to\_check \ = \ \{s_j \in S \quad \text{if} \ j \equiv i \mod num\_threads\}$
         \State \Call{remove\_dominated\_thread}{$S, V, u, to\_check$}
    \EndFor
    \Statex
   \Return $nd\_shared, ud(nd\_shared)$
\EndProcedure
\Statex
\Procedure{remove\_dominated\_thread}{$S, V, ud, to\_check$}
    \State $nd\_local \  = \ S$  \Comment{set of non-dominated strategies}
    \While{true}
        \State $si \ = \  to\_check\text{.get\_next\_schedule() }$ 
        \State $si\_gte \ = \ \{s_j \in to\_check  \quad \text{if} \ ud(s_i, v) \geq ud(s_j, v) \ \forall v  \in V \}$
        \State $si\_gt \ = \ \{s_j \in to\_check  \quad \text{if} \ \exists v \in V \text{s.t.}\ ud(s_i, v) > ud(s_j, v) \}$
        \Statex
        \If{$|to\_check| = 0$} \Comment{break when no more schedules to check}
            \State \textbf{break}
        \EndIf
        \Statex
        \If{\Call{sync}{$ $}}
            \State \Call{acquire}{$nd\_shared.\text{lock}$}
            \State  $nd\_shared \ = \ nd\_shared \cap nd\_local$
            \State $nd\_local \ = \ nd\_shared$
            \State $to\_check= \ \Call{prune}{to\_check, ud, nd\_local }$
        \EndIf
    \Statex
    \EndWhile
    \State \Call{acquire}{$nd\_shared.\text{lock}$}
    \State  $nd\_shared \ = \ nd\_shared \cap nd\_local$
    
    \Statex
    \Return
\EndProcedure
\end{algorithmic}
\end{algorithm*}

==> tables/prisoners.tex <==
\begin{table}
\centering
\begin{tabular}{l c c} 
 \toprule
  & \textbf{Confess} & \textbf{Cooperate}  \\ 
 \midrule
 \textbf{Confess}   & -3, -3 & 0, -5  \\ 
 \textbf{Cooperate} & -5, 0 & -1, -1  \\
 \bottomrule
\end{tabular}
\caption{Payoffs for the Prisoners Dilemma game.}
\label{table:prisoner}
\end{table}

==> tables/two_tables.tex <==
\input{tables/d_br_schedules}
\input{tables/randomized_best_response}

==> text/Acknowledgements.tex <==
\section{Acknowledgements}
Not sure if we have anything to put here?

==> text/Availability.tex <==
\section{Availability}

Sharing the samples directly as part of this publication would violate the agreement that we made in order to gain access to the dataset, so we do not include the dataset as part of this publication. If one wished to gain access to the for verification purposes, they could do so by filling out an academic research request here~\cite{vtaccess}, and requesting access to the downloadable resource.

\begin{itemize}
    \item Here is where we can include information about artifacts from our paper, so that others can recreate our findings.
    \item Where artifacts can be found.
    \item Explain how to use any artifacts.
\end{itemize}

